EADReg: Probabilistic Correspondence Generation with Efficient Autoregressive Diffusion Model for Outdoor Point Cloud Registration

Diffusion models have shown the great potential in the point cloud registration (PCR) task, especially for enhancing the robustness to challenging cases. However, existing diffusion-based PCR methods primarily focus on instance-level scenarios and struggle with outdoor LiDAR points, where the sparsity, irregularity, and huge point scale inherent in LiDAR points pose challenges to establishing dense global point-to-point correspondences. To address this issue, we propose a novel framework named EADReg for efficient and robust registration of LiDAR point clouds based on autoregressive diffusion models. EADReg follows a coarse-to-fine registration paradigm. In the coarse stage, we employ a Bi-directional Gaussian Mixture Model (BGMM) to reject outlier points and obtain purified point cloud pairs. BGMM establishes correspondences between the Gaussian Mixture Models (GMMs) from the source and target frames, enabling reliable coarse registration based on filtered features and geometric information. In the fine stage, we treat diffusion-based PCR as an autoregressive process to generate robust point correspondences, which are then iteratively refined on upper layers. Despite common criticisms of diffusion-based methods regarding inference speed, EADReg achieves runtime comparable to convolutional-based methods. Extensive experiments on the KITTI and NuScenes benchmark datasets highlight the state-of-the-art performance of our proposed method. Codes will be released upon publication.

==> sec/0_abstract_previous_version.tex <==
% %%%%%%%%% ABSTRACT
% \begin{abstract}
% Reactive mobile manipulation, which requires the robot's base to keep in motion when another high-level task is under operation. Facing such challenging characteristics, current works generally introduce many handcrafted environment-targeted modules. Despite the fantastic performance attained by prior approaches, it's hard for them to generalize, which hinders other researchers to follow. In this paper, without heavy design work, we propose a novel method for the robot to perceive and act accurately in an end-to-end manner, which utilizes the Visual Language Model (VLM) to generate the affordance 
% guidance and introduces a conditional reinforcement learning framework to study the accurate action planning based on real-time observations. 
% The remarkable experiments result in simulation and realistic environments demonstrate the effectiveness of our proposed method and superiority compared with others. 
% Video and Code are available at: \textcolor{blue}{XXXXX}.
% \end{abstract}

% %%%%%%%%% BODY TEXT
% \section{Introduction}
% \label{sec:intro}



% %Reference paper
% %T Target-referenced Reactive Grasping for Dynamic Objects
% %O On-The-Go Robot-to-Human Handovers with a Mobile Manipulator
% %A An Architecture for Reactive Mobile Manipulation On-The-Move
% %C Learning Human-to-Robot Handovers from Point Clouds

% In industrial scenarios, work with reactive mobile manipulation, like goods handling in the warehouse, requires workers to finish tasks fast and accurately. Robots are expected to be able to assist humans in completing these kinds of work, which will relieve the stress of people working in such labour-intensive environment. The main research concern of aforementioned case is how to guarantee robots' working effectiveness and successful interaction with humans. 

% The most critical challenge of manipulation on the move, is the favorable coordination between robot's base motion and high-level operation\{\textcolor{blue}{citecitexxx}\}. Prior researches generally decouple the mobile manipulation into two independent sub-tasks\{\textcolor{blue}{citecitexxx}\}, namely navigation and planning, in each task robot only pays attention to either base or arms controller. But in this case, the time effect of finishing a single task is totally omitted. Recently, by introducing complicated handcrafted control modules successes on mobile manipulation have been achieved\{\textcolor{blue}{citecitexxx}\}.
% However, these parametric modules are tightly related to the hardware, it reduces the reproducibility of the proposed methods to some extent.

% Meanwhile, conducting experiments on dynamic human robot interaction requires precise human modeling in simulation environment, which is intricate to collect\{\textcolor{blue}{citecitexxx}\}, leading to development difficulty in this area. Many works try to construct their own interaction dataset and demonstrate the effectiveness of the proposed method\{\textcolor{blue}{citecitexxx}\}. But due to the scale of training data, it's hard for them to generalize scenarios beyond training setting.
% Besides, researches on dynamic human robot interaction are mostly conducted between the human agent and the fixed robot\{\textcolor{blue}{citecitexxx}\}, which is quite different from the real-life interaction scene.


% In this paper, we aim to propose an effective method which can solve the coordination problem and implement dynamic interaction simultaneously. Note that interaction between human and robot contains numerous manners, in this paper we only focus on a common but nontrivial setting, namely human robot handovers.

% Unlike previous researches, instead of introducing complex module design, we abide by an end-to-end training paradigm, makes it much easier to follow and reproduce.
% In particular, based on the latest large scale handover simulation dataset "Handover-Sim"\{\textcolor{blue}{citecitexxx}\}, we develop a \{\textcolor{red}{xxxxxxx}\} reinforcement learning (RL) framework. Compared with other handover tasks, we propose to study an novel paradigm, in which the robot and human are moving contemporarily, which is much more challenging than others. In order to accelerate the rate of convergence and improve the exploration efficiency, we introduce 3D affordance map to constrain the action space of robot's arms. Constraint action space in contrast to arbitrary exploration, help robot to highlight the location of key object and avoid meaningless action. In short, RL only start when the robot perceive the \{\textcolor{red}{credible affordance}\}. Previous work mainly reasons object affordance via training a parametric modules with supervised label\{\textcolor{blue}{citecitexxx}\}, which limits the generalization towards unseen object.
% Inspired by the development of large vision language models (VLM), which have demonstrated their abilities in scene understanding\{\textcolor{blue}{citecitexxx}\}, we view affordance reasoning as the understanding result output by VLM. Based on this assumption,the robot first plans its trajectory towards potential handover object, according to the generated 3D affordance map. Once the value of the observed affordance \{\textcolor{red}{camera location still remain unclear}\} has reached pre-defined threshold, the robot start to explore and study the accurate handover paradigm via RL. Furthermore, we design a RL \{\textcolor{red}{framwork,that....}\}

% \{\textcolor{red}{We conduct experiments to demonstrate the effectiveness of affordance map generated by VLM as prior knowledge. We then present how
% our RL framework can learn to complete stably handover task.
% We provide an extensive ablation, revealing the superiority of our proposed method compared to others.

% Our contributions can be summarized as follows: 
% i) We introduce VLM to generate credible affordance map as helpful prior knowledge. ii) We propose an RL-based framework to study stably handover paradigm.
% iii) We conduct extensive experiments both in simulated and realistic environment. 
% Otherwise, we release the code, which is available at xxxx.}\}


\begin{abstract}
\label{abs}
% Previous Outdoor point cloud registration methods com-
% monly suffer from keypoint detection error in sparse key-
% point matching, and rely on outlier rejection modules due
% to inaccurate correspondence estimation. To tackle these
% challenges, we propose a probabilistic outdoor LiDAR reg-
% istration method, converting sparse keypoint matching into
% probability based outlier detection and local correspon-
% dence generating. Specifically, we first extract features
% based on the multi-layer SE(3)-invariant backbone, Subse-
% quently, instead of learning based outlier mask we intro-
% duce Gaussian mixture models (GMMs) to predict each . To
% establish correspondences between distributions, we match
% various GMMs based on the Wasserstein distance. Within
% the matched GMM pairs, we then sample points to predict
% point-level optimal correspondence matrices. Compared to
% previous keypoint-based methods, our probabilistic method
% has strong robustness to outliers. Extensive experiments on
% the KITTI and Nuscenes benchmark datasets demonstrate
% the state-of-the-art performance of our proposed method.
% Previous Outdoor point cloud registration methods commonly suffer from keypoint detection error in sparse keypoint matching, and rely on outlier rejection modules due to inaccurate correspondence estimation. To tackle these challenges, we propose a probabilistic outdoor LiDAR registration method, converting sparse keypoint matching into probability based outlier detection and local correspondence generating. Specifically, instead of introducing learning based outlier masks we utilize Gaussian Mixture Models (GMMs) to detect and reject the outlier clusters. Subsequently, To establish accurate correspondences between point cloud pairs, we propose a noval framework named \textbf{Lo}cal \textbf{Co}rrespondence \textbf{Di}ffusion in-the-\textbf{L}oop to generate reliable point correspondence between source and target point cloud. Compared to previous keypoint-based methods, our probabilistic method present superior performance, extensive experiments on the KITTI and Nuscenes benchmark datasets demonstrate the state-of-the-art performance of our proposed method.

% Previous outdoor point cloud registration methods commonly suffer from keypoint detection errors in sparse keypoint matching and rely on outlier rejection modules due to inaccurate correspondence estimation. To tackle these challenges, we propose a probabilistic outdoor LiDAR registration method that converts sparse keypoint matching into probability-based outlier detection and local correspondence generation. Specifically, instead of using learning-based outlier masks, we utilize \textbf{G}aussian \textbf{M}ixture \textbf{M}odels (\textbf{GMMs}) to detect and reject outlier clusters.

% To establish accurate correspondences between point cloud pairs, we propose a novel framework named \textbf{Lo}cal \textbf{Co}rrespondence \textbf{Di}ffusion in-the-\textbf{L}oop (\textbf{EADReg}) 
% to generate reliable point correspondences between source and target point clouds,
% unlike previous diffusion-based registration method focusing on constructing powerful condition features, we design the diffusion-in-the-loop paradigm which makes sure the generated correspondence subject to the real translation. Compared to previous keypoint-based methods, our probabilistic method demonstrates superior performance. Extensive experiments on the KITTI and NuScenes benchmark datasets showcase the state-of-the-art performance of our proposed method.

%abs:
%被忽视的问题、问题来源、重要性、提出新方法
%intro：
% ●.指出当前领域的发展情况，在实际应用中遇到了什么问题。
% ●.当前领域的代表工作有什么，他们都是如何迭代改进的，总结这些方法的不足，说明他们并没有认识到本文中提出的问题。
% ●.解决这个问题我们提出了什么结构，介绍结构的组成。并且指出本文的结构跟以往的研究工作有何不同，做了哪些改进，并且指出每个改进是如何克服之前存在的问题的，改进后带来的效果又是什么。
% ●.总结论文对当前领域做出的贡献
With the development of generative schemes, diffusion models have attracted researchers to introduce them into point cloud registration (PCR) tasks. However, existing diffusion-based PCR methods primarily focus on instance-level scenarios and struggle in outdoor LiDAR scenarios. We assume that the intrinsic bottleneck problem arises from the sparsity and low discriminability of LiDAR point cloud characteristics, which pose challenges in finding the best point-to-point (P2P) correspondences. \ma{[assume is not suited to claim a finding, change to `argue'?]}

This study introduces a novel framework, EADReg, for efficient and robust global registration of LiDAR point clouds, 
% named Local Correspondence with \textbf{L}oop \textbf{S}ampling \textbf{D}iffusion (\textbf{EADReg}) for outdoor LiDAR point cloud registration. 
EADReg follows the coarse to fine registration paradigm,
In the coarse stage, we reject the outlier point clusters through Bi-directional Gaussian Mixture Models Matching Module (BGMM) to obtain purified point cloud pairs. BGMM establishes corresponding relationship between the GMMs of the source and target point clouds. The points, contained in a GMM which can not find its counterpart will not be considered during registration.
After that, we can easily perform reliable coarse registration based on the filtrated points' features and primitive geometric information. \ma{[do not need so many details in abstract (too long for now), `proposed module + aim' is enough]}

% Specifically, in the coarse stage, we utilize Gaussian Mixture Models ({GMMs}) to model the input points and reject outlier clusters.
% Previous diffusion-based PCR models, treating diffusion as a powerful regressor to predict the reliable translation and rotation vectors.
In the fine stage, we regard diffusion-based PCR as an autoregressive process and
% follow autoregressive inference manner to
generate a robust point correspondence matrix between two adjacent sampling steps, the generated correspondences are decomposed into translation and rotation to warp the input source points, which will constitute the next step's source point.
Additionally, although diffusion-based methods are roundly criticized for the low inference speed, we also demonstrate that the running time of EADReg is comparable with the convolutional-based methods. 
% Specifically, the generated correspondences are decomposed into translation and rotation to warp the input source points, which will constitute the next frame's source point.
% We also demonstrate that the Sinkhorn algorithm is effective to construct the required correspondence ground truth. 
Compared to previous methods, our probabilistic approach demonstrates superior performance. Extensive experiments on the KITTI and NuScenes benchmark datasets highlight the state-of-the-art performance of our proposed method. The code will be released in the github. \ma{[The code and pretrained models will be released as opensource.]} 

\ma{[I think the correct logic at the end of the abstract (from "Additionally, ..") should be: Extensive experiments validate SOTA performance and lower running time compared to convolutional-based methods]}

\end{abstract}

==> sec/1_intro_previous_version.tex <==

\section{Introduction}
\label{sec:intro}

% Point cloud registration in outdoor environments is an important technique for global localization [citations], SLAM [citations], and navigation [citations] in robotics and autonomous driving applications. It discovers the point-level relationship between two LiDAR frames to compute their 6-DOF rigid transformation. To this end, point descriptors are first extracted through either hand-crafted methods [citations] or learning-based [citations] approaches, and then a correspondence matrix is generated to facilitate finding the spatial relationship between nonhomologous point clouds, i.e., rotation and translation [don't know whether accurate]. Considering the existing large-scale point cloud registration works, much effort has been devoted to enhancing the performance of front-end point descriptors such as [algorithm name citations]. However, the reliability degree of such feature extractor always bring up the increasing computational complexity and slow convergence speed which hinders their real-world applications. 
% The back-end rigid transformation estimation is nontrivial to achieve by ICP or ... [citations], however, the estimation precision for outdoor scenarios can not be guaranteed because of the sparsity of the outdoor lidar point cloud scene. To this end, we argue that attentions should be focused on concise front-end descriptors filtrate and the reliable back-end rigid transformation estimation.
%---
% Point cloud registration(PCR) in outdoor environments is a fundamental process for global localization[citations], SLAM[citations], and navigation in robotics and autonomous driving applications[citations]. PCR aims to compute the six degrees of freedom (6-DOF) rigid transformation between two LiDAR frames. This process involves extracting reliable point features using either hand-crafted methods or learning-based approaches, introducing efficient alignment algorithm to establish the accurate point-to-point(P2P) correspondence and calculating the parameters of the transformation matrix[citations] through the variants of the singular value decomposition (SVD). 

% Recent years, much effort in existing methods has focused on enhancing the performance of point descriptors. GeoTransformer[citations] introduces PointTransformer architecture into PCR tasks and encodes the high-level intra and inter point features through the attention mechanism. DiffPCR[citations] construct a powerful Transformer-based feature extract network to ensure the generation quality. Roreg[citations] proposes an oriented descriptor which has both rotation equivariance and rotation-invariance. However, the reliability of such powerful feature extractors often leads to increased computational complexity and slower convergence speeds, hindering their real-world applications.

% The establishment of the accurate P2P correspondence can be presented as the correspondence matrix by using metrics such as cosine similarity. CofiNet[citations] Lepard[citations] and GeoTransformer[citations] further introduce Optimal Transport(OT) to eliminate the uncertainty within the coarse correspondence matrix. Without establishing the correspondence matrix, HRegNet[citations] construct the P2P correspondence by aggregating the neareast target points of source points and achieve excellent performance. However, due to the sparsity and low discriminability of outdoor LiDAR point clouds, the registration results always suffer from the mismatching entries in correspondence. 
% Recently, the novel generative schemes \textbf{D}enoising \textbf{D}iffusion \textbf{P}robabilistic \textbf{M}odels(\textbf{DDPMs}) have been applied to multiple domains such as Image and Video Generation, Segmentation and object motion prediction[citations] and present solid ability to generate the realistic predictions from the standard Gaussian noise. Building on these advancements, recent studies start to introduce diffusion for images matching tasks. DiffMatch first introduces diffusion to explicitly model the matching filed distribution with images. A few attempts have been made to extend diffusion into point cloud registration[citations] for accurate dense correspondence generation and translation matrix regression. DiffReg[citations] introduces diffusion as a reliable solver which directly regress the transformation parameters. DiffReg[citations] utilizes OT to construct the ground truth as supervision and forces the diffusion to generate the reliable Correspondence. But few of them presents generalizability towards outdoor scenarios. 

% In order to tackle the aforementioned issues, we propose a novel probabilistic method named \textbf{Lo}cal \textbf{Co}rrespondence \textbf{Di}ffusion in-the-\textbf{L}oop (\textbf{EADReg}) for outdoor LiDAR point cloud registration, which combines the GMMs-based front-end outlier cluster rejection with the Diffusion based back-end rigid transformation estimation. The overall framework are displayed in the Fig. [citations]. Specifically, We first downsample the point cloud pairs and extract their corresponding descriptors through hierarchical networks as HRegNet[citations]. Instead of introducing amount of parameters to learn to reject outlier points, we use GMMs to model the downsampled superpoints and efficient reject the outlier cluster according to the designed geometric metrics. Subsequently, in order to generate the reliable correspondence matrix, inspired by traditional registration method like ICP(Iterative Closest Point), we treat the generation process as a repetitive loop architecture. For each step in the loop, EADReg only pays attention to the local region of the source points which efficient reduce the training pressure of EADReg. During training, the generated correspondence matrix will be forced to learn the \textbf{posterior} distribution of ground truth correspondence matrix and abide by the real transformation. The loop architecture enables EADReg to repetitive refine the input source points using derived transformation from last step and generate more robust correspondence matrix.
%----
% the correspondence residual map is obtained by comparing the coarse correspondence matrix and the ground-truth one. It is then gradually corrupted into a standard Gaussian distribution step by step in a diffusion process, after which a convolution-based denoising model is proposed learning to reverse this process. Therefore, we achieve a correspondence refinement process to capture the variation imposed on the coarse correspondence matrix in the inference process. Note that the proposed refinement can be regarded as an alternative implicit iteration process at the feature correspondence level compared to the traditional explicit iteration at the spatial distance level [citation]. In addition, we further propose using fine-grained point features as the condition for the denoising process, which lets the denoising network be aware of the spatial and feature distribution of input laser points simultaneously. Our proposed xxx exhibits good point cloud registration performance and strong robustness across different large-scale environments due to the powerful generation ability inherent in the diffusion-based scheme.


% Therefore, to address the aforementioned issues in both front-end and back-end algorithms, we argue that attention should be focused on refining front-end descriptors and introducing a novel reliable back-end rigid transformation estimation algorithm.

Point cloud registration (PCR) in outdoor environments is a fundamental process for global localization~\cite{Elbaz_2017,Pomerleau_2015,Sun_2022,Xie_2021}, SLAM~\cite{Cattaneo_2022,Hitchcox_2020,Jiang_2023_nav}, and navigation in robotics and autonomous driving applications~\cite{Miao_2016,Kim_2019,Pomerleau_2015}. PCR aims to compute the six degrees of freedom (6-DOF) rigid transformation between two LiDAR frames. This process involves extracting reliable point features using either hand-crafted methods or learning-based approaches, introducing efficient alignment algorithms to establish accurate point-to-point (P2P) correspondences, and calculating the parameters of the transformation matrix through variants of the singular value decomposition (SVD).

% Point cloud registration aims to find the optimal translation matrices to align a Point cloud registration aims to find the optimal translation matrices to align a point cloud registration aims to find the optimal translation matrices 1to align a Point cloud registration aims to find the optimal translation matrices to align a 

\begin{figure}
\centering
\includegraphics[scale=0.24]{fig/head_figure_abbr.pdf}
% \vspace{-0.2cm}
\caption{\ma{[all important elements in each figure of this paper such as ``intra registration'' here should be mentioned in the main text. (Maybe you have not revised this figure from the previous paper~)]}}
\label{fig.loopdiff}
	% \vspace{-5mm}

\end{figure}

In recent years, much effort in existing methods has focused on enhancing the performance of point descriptors. GeoTransformer~\cite{GeoTransformer} introduces the PointTransformer architecture into PCR tasks, encoding high-level intra- and inter-point features through the attention mechanism. DiffusionPCR~\cite{DiffusionPCR} constructs a powerful Transformer-based feature extraction network to ensure generation quality. Roreg~\cite{roreg} proposes an oriented descriptor that has both rotation equivariance and rotation invariance. However, the reliability of such powerful feature extractors often leads to increased computational complexity and slower convergence speeds, hindering their real-world applications.

The establishment of accurate P2P correspondences can be presented as a correspondence matrix using metrics such as cosine similarity. CofiNet~\cite{Cofinet}, Lepard~\cite{Lepard}, and GeoTransformer~\cite{GeoTransformer} further introduce Optimal Transport (OT)~\cite{Optimaltransport} to eliminate the uncertainty within the coarse correspondence matrix. Without establishing the correspondence matrix, HRegNet~\cite{HRegNet} constructs the P2P correspondences by aggregating the nearest target points of source points, achieving excellent performance. \ma{[what's the contribution of this paragraph on introducing `our work'? Neither limitation nor motivation is provided here.]}
% However, due to the sparsity and low discriminability of outdoor LiDAR point clouds, the registration results always suffer from mismatching entries in correspondence.

Recently, novel generative schemes, \textbf{D}enoising \textbf{D}iffusion \textbf{P}robabilistic \textbf{M}odels (\textbf{DDPMs}), have been applied to multiple domains such as image and video generation, segmentation, and motion prediction~\cite{Zhang_2023,ho2022imagen,Jiang_2023}. They demonstrate solid ability to generate realistic predictions from standard Gaussian noise. Building on these advancements, recent studies have started to introduce diffusion for image matching tasks. DiffMatch~\cite{diffmatch} first introduces diffusion to explicitly model the matching field distribution within images. A few attempts have been made to extend diffusion into point cloud registration~\cite{DiffusionPCR,diffpcr,she2024pointdifformer,se3diff} for accurate dense correspondence generation and translation matrix regression. DiffusionPCR~\cite{DiffusionPCR} introduces diffusion as a reliable solver that directly regresses the transformation parameters. DiffPCR~\cite{diffpcr} utilizes optimal transport(OT) to construct the ground truth as supervision and forces the diffusion to generate reliable correspondences. However, few of these methods present generalizability towards outdoor scenarios. We assume that the intrinsic bottleneck problem arises from the sparsity and low discriminability of LiDAR point cloud characteristics, which pose challenges in finding the best point-to-point (P2P) correspondences.

To tackle the aforementioned issues, we propose a novel probabilistic method named \textbf{E}fficient \textbf{A}utogressive \textbf{D}iffusion (\textbf{EAD}) for outdoor LiDAR Point Cloud \textbf{Reg}istration, which combines the GMMs-based front-end outlier cluster rejection with the diffusion-based back-end robust P2P correspondence estimation. The overall framework is displayed in Fig.~\cite{}. Specifically, we follow the coarse-to-fine paradigm and downsample the point cloud pairs through hierarchical networks as HRegNet~\cite{HRegNet}. In order to perform reliable coarse registration, the harmful noisy point should be effectively removed. Unlike previous work~\cite{OMNet,UTOPIC,Rethinking_2023} introduce extra parameters to find outlier masks, we design the
\textbf{B}i-directional \textbf{G}aussian Mixture Models \textbf{M}atching \textbf{M}odule({BGMM}) to reject outlier points. BGMM first constructs GMMs based on the downsampled point cloud pair, then utilizes the GMMs' geometric features to establish corresponding relationship between the source and target point clouds. A natural idea is to remove the GMM which cannot establish bi-directional nearest neighborhood. However, due to the randomness of the probabilistic model, the bi-directional nearest neighborhood cannot be guaranteed.
We loose this strict rule by only removing the GMMs which is not the top-K nearest neighbor of its nearest neighbor. In this way, we can find the true outlier GMMs, and the points contained in this GMM will not be considered during registration.
After that, we can easily perform reliable coarse registration based on the purified points' features and primitive geometric information.

% we design the use GMMs to model the downsampled superpoints and efficiently reject outlier clusters according to designed geometric metrics.
Inspired by the diffusion-based temporal motion prediction methods~\cite{Tang_2024,BeLFusion,DiffusionPoser,Humor}, we 
% introduce the idea of registration history and 
rethink the diffusion-based PCR as an autoregressive process. During inference, 
% the source points will be dynamicly warped by the transformation,
the diffusion model will generate a robust point correspondence matrix between two adjacent sampling steps, the generated correspondences are decomposed into translation and rotation to warp the input source points, which will constitute the next step's source point.



% can separate each sampling step into several sequence frames and 
% introduce autoregressive diffusion paradigm to generate robust point correspondence matrix between adjacent two sequence frame, which means the current transformation is built on the previous transformation history. 
Specifically,
% to generate a reliable correspondence matrix, inspired by traditional registration methods like ICP (Iterative Closest Point), we treat the generation process as a repetitive loop architecture. 
for each frame, the generated correspondence matrix will be forced to learn the \emph{posterior} distribution of the ground truth correspondence matrix and be 
decomposed into translation and rotation to warp the input source points, which will constitute the next frame's source point. 
The transformation will be preserved in the history buffer, the final result can be derived from the sequential product of all the transformation in this buffer.
We also demonstrate that utilizing the Sinkhorn algorithm upon the Euclidean distance matrix can effectively construct the ground truth correspondence. \ma{[The introduction to the algorithm is too lengthy and should be more concise. I think it would be better to follow either a motivation+method flow or a method+problem-solved flow to give a brief overview of the method.]}

In order to achieve efficient generation, we show that only paying attention to the top-K nearest region of the source points instead of the global is enough to find the truly corresponding targets due to the reliable coarse registration, which significantly reduces the memory usage and achieves superior performance. 
% decomposed into transformation. The loop architecture enables EADReg to iteratively refine the input source points using derived transformations from the previous step, generating a more robust correspondence matrix.

Our proposed method exhibits the following favorable properties: \ma{[Why not directly claim contributions here? Maybe this style is not mainstream in CV papers]}

\textbf{Large Scale Generalizability}: Our method accurately registers outdoor large-scale point cloud pairs with arbitrary displacements and without any initialization.

\textbf{Autoregressive Registration Diffusion}: As far as we know, EADReg is the first regarding the single frame PCR as a sequence registration process. In this way, the training process can be constructed in the autoregressive diffusion paradigm.
and derive the final transformation step by step.

% and the final transformation can be derived from the registration history.
Due to the superior denoising property of DDPMs, our method is tolerant to perturbation which exists extensively in the outdoor LiDAR frames.

\textbf{Efficient Generation}: Benefiting from the reliable coarse registration, EADReg can directly find the truly corresponding target from the top-K nearest neighbor of the source points instead of the global targets. In this way, the computation speed can even be comparable with the convolution-based methods while maintaining the generation precision. 

\textbf{Superior Performance}: We demonstrate the advantages of our method over the state-of-the-art on general outdoor datasets such as KITTI and Nuscenes. Through extensive experiments and visible results, our proposed method showcases convincing performance surpassing previous methods.

